A New Upper Bound for the Traveling Salesman Problem in Cubic Graphs

We provide a new upper bound for traveling salesman problem (TSP) in cubic graphs, i.e. graphs with maximum vertex degree three, and prove that the problem for an $n$-vertex graph can be solved in $O(1.2553^n)$ time and in linear space. We show that the exact TSP algorithm of Eppstein, with some minor modifications, yields the stated result. The previous best known upper bound $O(1.251^n)$ was claimed by Iwama and Nakashima [Proc. COCOON 2007]. Unfortunately, their analysis contains several mistakes that render the proof for the upper bound invalid.

==> 4cycle.tex <==
      %\node[vertex] (a1) at (1,1.9) {};
      \node[vertex] (a2) at (0,0) {};
      \node[vertex] (a3) at (2.1,0) {};

      %\draw [->] (0.9,0.9) -- (0.7,0.7);
      %\draw [->] (1.7,0.9) -- (1.9,0.7);

      \foreach \ind in {2,3} {
        \input{4cycle-comp}
        \foreach \source/ \dest in {a\ind/e\ind, b\ind/f\ind}
          \path[edgef] (\source) -- (\dest);
      }


==> 5cycle.tex <==
      \node[vertex] (b) {};
      \node[vertex] (c) [below=of b] {};
      \node[vertex] (d) [below left=of c] {};
      \node[vertex,label=below:$y$] (e) [above left=of d] {};
      \node[vertex,label=left:$z$] (a) [above=of e] {};

      \node[] (f) [above=of a] {};
      \node[] (g) [above=of b] {};
      \node[] (h) [right=of c] {};
      \node[] (i) [below=of d] {};
      \node[] (j) [left=of e] {};


==> 6cycle-att.tex <==
      \node[vertex,label=left:$z$] (a1) at (0,0) {};
      \node[vertex,label=left:$z$] (a2) at (3.2,0) {};

      \foreach \ind in {1,2} {
        \input{6cycle-comp}
        \node[vertex,label=above left:$y$] (f\ind) [above left=of e\ind] {};
        \node[vertex,label=above:$x$] (e\ind) [left=of d\ind] {};
      }

      \foreach \source/ \dest in {}
        \path[edge] (\source) -- (\dest);
      \foreach \source/ \dest in {f1/l1, a1/g1, f2/l2, a2/g2}
        \path[edgef] (\source) -- (\dest);
      \foreach \source/ \dest in {e1/f1, a1/b1, f2/a2}
        \path[edgerem] (\source) -- (\dest);
      \foreach \source/ \dest in {f1/a1, d1/e1, b1/c1, a2/b2, e2/f2}
        \path[edgesel] (\source) -- (\dest);


==> 6cycle-branch-comp.tex <==
      \node[vertex, label=right:$z$] (b\ind) [right=of a\ind] {};
      \node[vertex] (c\ind) [below right=of b\ind] {};
      \node[vertex] (d\ind) [below left=of c\ind] {};
      \node[vertex] (e\ind) [left=of d\ind] {};
      \node[vertex] (f\ind) [above left=of e\ind] {};

      \node[vertex] (g\ind) [above=of a\ind] {};
      \node[vertex] (h\ind) [above=of b\ind] {};
      \node[vertex] (i\ind) [right=of c\ind] {};
      \node[vertex] (j\ind) [below=of d\ind] {};
      \node[vertex] (k\ind) [below=of e\ind] {};
      \node[vertex] (l\ind) [left=of f\ind] {};


==> 6cycle-branch.tex <==
\node[vertex, label=left:$y$] (a) {};
\newcommand{\ind}{} 
\input{6cycle-branch-comp}


==> 8cycle.tex <==
      \node[vertex] (a) {};
      \node[vertex] (b) [right=of a] {};
      \node[vertex] (c) [right=of b] {};
      \node[vertex] (d) [below=of c] {};
      \node[vertex] (e) [below=of d] {};
      \node[vertex] (f) [left=of e] {};
      \node[vertex,label=below:$y$] (g) [left=of f] {};
      \node[vertex,label=right:$z$] (h) [above=of g] {};

      \node[] (i) [left=of a] {};
      \node[] (j) [above=of b] {};
      \node[] (k) [right=of c] {};
      \node[] (l) [right=of d] {};
      \node[] (m) [right=of e] {};
      \node[] (n) [below=of f] {};
      \node[] (o) [left=of g] {};
      \node[] (p) [left=of h] {};


==> chain.tex <==
      \node[vertex] (a) {};
      \node[vertex] (b) [below right=of a] {};
      \node[vertex,label=right:$y$] (c) [above right=of b] {};
      \node[vertex,label=right:$z$] (d) [below right=of c] {};
      \node[vertex] (e) [above right=of d] {};
      \node[vertex] (f) [below right=of e] {};

      \node[] (h) [below=of b] {};
      \node[] (i) [above=of c] {};
      \node[] (j) [below=of d] {};
      \node[] (k) [above=of e] {};


==> single-4cycle.tex <==
\node[vertex] (a) {};
\newcommand{\ind}{} 
\input{4cycle-comp}


==> triangle.tex <==
\node[vertex,label=right:$x$] (x\ind) [below=of a\ind] {};
\node[vertex,label=right:$y$] (y\ind) [below right=of x\ind] {};
\node[vertex,label=left:$z$] (z\ind) [below left=of x\ind] {};

\node[] (b\ind) [below right=of y\ind] {};
\node[] (c\ind) [below left=of z\ind] {};

